Multi-resolution Time-Series Transformer for Long-term Forecasting

The performance of transformers for time-series forecasting has improved significantly. Recent architectures learn complex temporal patterns by segmenting a time-series into patches and using the patches as tokens. The patch size controls the ability of transformers to learn the temporal patterns at different frequencies: shorter patches are effective for learning localized, high-frequency patterns, whereas mining long-term seasonalities and trends requires longer patches. Inspired by this observation, we propose a novel framework, Multi-resolution Time-Series Transformer (MTST), which consists of a multi-branch architecture for simultaneous modeling of diverse temporal patterns at different resolutions. In contrast to many existing time-series transformers, we employ relative positional encoding, which is better suited for extracting periodic components at different scales. Extensive experiments on several real-world datasets demonstrate the effectiveness of MTST in comparison to state-of-the-art forecasting techniques.

==> sections/apendix.tex <==
\newpage
\section{APPENDIX}
\subsection{Experimental Details}
\subsubsection{Datasets}
describe the dataset breively, list all links of the datasets.

\subsubsection{Implementation Details}

\subsection{Full benchmark of multivatiate forecasting}


\subsection{More Ablation Study}

\subsubsection{Look back window}



% \subsection{Robustness analysis}



==> sections/old_version/experiments.tex <==

\section{EXPERIMENTS}
\label{sec:exp}
datasets, baselines, experimental setup, hyperparameters (details in appendix), discussion of the main result.

Ablation study 1: effect of cutting branches from MTST.

Ablation study 2: comparison between MTST with no PE, MTST with Absolute PE, and MTST (relative PE).

visualization: multi-scale forecasts from real datasets. 

(if result is available), study the effect of look-back window for MTST.

\subsection{Benchmarking MTSTs}

\subsubsection{Datasets}
% \st{In our experiments, we utilized eight publicly available},
We evaluate the performance of our proposed MTST on seven extensively-utilized
public benchmark datasets: ETTh1, ETTh2, ETTm1, ETTm2, Weather, Traffic, and Electricity ~\citep{wu2021AutoformerDecompositionTransformers}. 
We follow the experimental setting of  PatchTST~\citep{nie2023TimeSeriesWorth} that
the dataset is split into training, validation, and test sets with the ratio of $6{:}2{:}2$ for four ETT datasets and $7{:}1{:}2$ for the remaining datasets.
Detailed statistics of the datasets is in Table.~\ref{tab:datasetStat}.
It is worth mentioning that the results from larger datasets (Weather, Traffic, and Electricity) 
shall be highlighted since they are more stable and less susceptible to overfitting.

% The datasets consist
% of variables with diverse characteristics, and they are sampled at different frequencies, ranging from every 10 minutes to every 1 week, resulting in varying temporal dependencies among them.


\begin{table}[htbp]
    \centering
    \scriptsize
    \setlength{\tabcolsep}{2pt}
    \begin{tabular}{c|ccccc}
    \toprule
Datasets & ETTh1/2 & ETTm1/2 & Traffic & Electricity & Weather  \\ 
    \midrule
Variates & 7 & 7 & 862 & 321 & 21 \\
Timesteps & 17,420 & 69,680 & 17,544 & 26,304 & 52,696  \\
Granularity &1 hour &5 min &1 hour &1 hour &10 min \\
    \bottomrule
    \end{tabular}
    % \begin{tabular}{l|ccc}
    % \toprule
    %     Datasets & ETTh1/2 & ETTm1/2 & Traffic \\ \midrule 
    %     Variates & 7 & 7 & 862 \\ 
    %     Timesteps & 17,420 & 69,680 & 17,544 \\ 
    %     Granularity & 1hour & 5min & 1hour \\ \midrule
    %     Datasets & Electricity & Weather & ILI \\ \midrule
    %     Variates & 321 & 21 & 7 \\ 
    %     Timesteps & 26,304 & 52,696 & 966 \\ 
    %     Granularity & 1hour & 10min & 1week \\ \bottomrule
    % \end{tabular}
    \caption{The statistics of datasets in the experiments}
    \label{tab:datasetStat}
\end{table}




\subsubsection{Baselines and Experimental Setup}

To evaluate our model, we conduct two sets of experiments with two mainstream experimental setups in time-series forecasting.

In the first experiment, 
we follow the experimental setup in ~\citet{nie2023TimeSeriesWorth}, where the look-back window $L=336$ and the prediction horizon $T\in\{96, 192, 336, 720\}$.
We compare to the state-of-the-art TST -- PatchTST~\citep{nie2023TimeSeriesWorth}; a competitive non-transformer-based model -- DLinear~\citep{zeng2023AreTransformersEffective}; and three popular timestamp-based TSTs -- 
FEDformer~\citep{zhou2022FEDformerFrequencyEnhanced}, Autoformer~\citep{wu2021AutoformerDecompositionTransformers}
and Informer~\citep{zhou2021InformerEfficientTransformer}.
We collect the baseline results from \cite{nie2023TimeSeriesWorth}.
Note that the results for timestamp-based TSTs are chosen the best from six potential look-back windows $L\in \{24, 48, 96, 192, 336, 720\}$ while the other models are based on $L=336$.


In the second experiment, we consider the \textit{de facto} standard setup for TSTs, where the look-back window $L=96$ and the prediction horizon $T\in\{96, 192, 336, 720\}$.
Under this setup, 
we compare to a recent patch-based TSTs -- Crossformer~\citep{zhang2022crossformerTransformerUtilizing};
the latest multiscale TSTs -- Scaleformer~\cite{shabani2023Scaleformer}; two multiscale convolution-based models \mlh{to reword after discussion} -- MICN~\cite{wang2023MicnMultiscaleLocal}, Timesnet~\cite{wu2022TimesnetTemporal2dVariation}.
Besides, we reproduce PatchTST with $L=96$ for reference.

\mlh{to add scaleformer and timesnet to related works.}


\subsubsection{Hyperparameters}

% In MTST, 
% $\mathbf{x} \in \RR^L$  will be first patched at different resolutions at each branch. MTST contains 2 branches and 2 layers. 

% \mlh{how MTST works shall be moved to \textbf{methodology}; \\
% \textbf{``2 branches and 2 layers...''} shall be deleted; they are hyperparameters; The detailed hyparameter choices shall be hidden in the appendix.
% }

% At each layer, the patch length and stride is $P = \{16, 96\}$ and $S = \{8, 48\}$ for the 2 branches. The number of patches is calculated by $K = \frac{L-P}{S}+1$. Then the patches would be linear mapped to $\RR^{K \times D}$, where $D = 128$.
\mlh{To update after getting the final results}
The feed forward network in Transformer encoder block consists of 2 linear
layers with GELU activation function: one projecting the hidden
representation $D=128$ to a new dimension $F=256$, and another layer that project it back to
$D$. 
% The Hyperparameters of MTST is shown in Table.\ref{MTST_hp}.
Dropout with probability 0.2 is applied in the encoders for all experiments.
For training, we utilize the Adam optimizer with an initial learning rate ranging at $1e^{-4}$.
% \begin{table}[h!]
%     \centering
%     \caption{Hyperparameters of MTST}
%     \label{tab:hyper_pyramid}
%     \begin{tabular}{c|c}
%     \toprule
%        % &  Electricity, Traffic, Weather \\ \midrule
%        Patch Length ($P$)  & [16, 96]    \\
%        Patch Stride ($S$) & [8, 48]  \\
%        \bottomrule
%     \end{tabular}
%     \begin{adjustwidth}{1cm}{1cm}
%     % $\mathbf{x} \in \RR^L$  will be first patched $\RR^{K \times \frac{L}{K}}$, then linear mapped to $\RR^{K \times D}$. 
%     % Afterward, the total length $K\cdot D$ will not be changed with different $K$ at the following layers.
%     \end{adjustwidth}
%     \label{MTST_hp}

% \end{table}

% \subsection{Evaluation and baselines}




% We choose state-of-the-art (SOTA) Transformer-based baseline methods, including PatchTST, Crossformer, ScaleFormer, FEDformer. MICN, DLinear, FEDformer.

% \mlh{Dlinear is not a transformer}
 

% We obtained the results of PatchTST, DLinear, Fedformer from \cite{nie2023TimeSeriesWorth}.
% % \st{The results
% % for PatchTST were reproduced.}

% % In cases where results are not available, we conducted experiments using the optimal hyperparameters as presented in the original papers. \soumya{If results are not available, how do you know which hyperparameters are 'optimal'? 'as presented in the original papers' does not make sense to me.}
% % \yitian{like $D$ or number of transformer layers. We can delete it.}
% In particular, for a fair comparison, we did not fix the input length to 96, as recent studies have highlighted the significance of optimal input lengths for method performance.


% \lm{[liheng: already mention this in problem statement. No need to duplicate]}
% \lm{Following the standard pipeline in previous works, 
% we utilize the Mean Squared Error (MSE) 
% as the metrics for forecasting.
% Besides, we also include the Mean Absolute Error (MAE) for reference.}
% % metrics as quantitative
% % measures of forecasting accuracy.

% \lm{Results shown on the table are corresponding to the best for each model across hyperparameter choices.}


\subsubsection{Experimental Results}



% The results are shown in table.~\ref{tabel:mtst}. 
% We can see that the newly proposed structural configuration consistently demonstrates a noteworthy trend of small yet discernible improvements in performance across all datasets. This observation underscores the robustness and reliability of our model's enhanced capabilities. 

% Figure.5 serves as compelling evidence that our multiscale structure, with multiple layers, excels at capturing diverse patterns within the data. Each layer within the architecture demonstrates a unique ability to capture and represent distinct temporal features, thereby highlighting the efficacy of our model in capturing a wide range of information.

% Figure.6 visualizes the attention map on an example dataset. It shows that the L2 attention mechanisms proves advantageous in the task of identifying periodic patterns. By applying L2 attention, our model gains the ability to capture and emphasize the underlying periodic components, thereby enhancing its performance in detecting and characterizing recurring temporal behaviors. Simultaneously, the incorporation of relative positional encoding (RPE) further enhances our model's ability to capture periodicity within time series data. Relative PE not only aids in identifying periodic patterns but also makes a valuable contribution to the overall score or performance metric, underscoring its significance in our approach.

% Since there is performance drop in Traffic dataset, we visualized the output of each layer in figure.~\ref{fig:iptst_traffic_720}. It shows that each layer does not capture different frequency as we expected, and most of the information are left for the residual layers. It demonstrates that the current max-pooling and interpolation design is not ideal. 

% We also did one experiment for not connecting the final residual back. The hypothesis is that if do not add it to the output, each layer would be forced to learn its own pattern. Figure.~\ref{fig:iptst_traffic_720_nores} shows that the each layer can learn some frequencies, but without the residual, we lost a lot of details, so the prediction on the peak is less accurate, resulting a higher MSE (0.519). However, we can see that the Layer 1 is learning daily pattern, Layer 2 is more like weekly pattern. Aftbaer removing the first 2 layers, the Layer 3 should be more focus on the peak, but with interpolation and max-pool, the output is more smooth. Therefore, I would just remove the interpolation for Layer 3 to see if we can get better predictions.

% \textbf{Boxplot on Traffic and Electrcity dataset}

% From Figure.7 and Figure.9, the box plot analysis provides evidence that the superior results consistently originate from each variate within the dataset. This observation underscores the robustness of our method, which exhibits consistent performance enhancements across most variates.

% For traffic dataset, upon examining each variate individually and plotting the comparison between predictions and errors, a noteworthy pattern emerges. It becomes evident that within the traffic dataset, the substantial performance improvement is mainly associated with the peak values. This observation underscores the significance of modeling and accurately capturing peak patterns for enhancing forecasting accuracy in the context of traffic data.

% Regarding to the electricity, the observation highlights two important patterns in the data and how MTST can capture them. Firstly, it's common to observe distinct patterns during weekends, often characterized by reduced electricity demand compared to weekdays. The visualization suggests that MTST is effective at capturing and modeling this specific weekend trend. For example, in Figure. 10 (b),  at around time step 450, MTST has more flat prediction, which is closer to the ground truth.  This ability to discern and adapt to weekly variations in consumption can lead to more accurate forecasts, as it accounts for the cyclic nature of electricity usage. Secondly, when we look into Figure. 10 (a), MTST shows the capacity to handle random noise effectively. Time series data, including electricity consumption, can be subject to various sources of noise and irregular fluctuations that make forecasting challenging. MTST's stability in the presence of such noise indicates that it can distinguish between underlying patterns and random fluctuations. This stability is crucial for maintaining the integrity of forecasts and preventing undue influence from transient noise.

% Overall, multiscale modeling leverages the hierarchical nature of time series data, enabling the forecasting model to capture a wide range of temporal patterns and adapt to various data dynamics. This adaptability and the ability to capturing both systematic patterns (e.g., weekend variations) and maintaining stability in noisy environments can lead to improved forecasting performance, making it a valuable approach.



% \begin{table*} 
% \centering
% \tiny
% \caption{Multivariate long-term forecasting results with MTST. Look back window $L=336$. We use prediction
% lengths $T \in \{24, 36, 48, 60\}$ for ILI dataset and $T \in \{96, 192, 336, 720\} $ for the others. The best
% results are in \textbf{bold} and the second best are {\ul underlined}. \soumya{write one sentence about how the improvement is computed. What metric are you using?}

% \label{tabel:mtst}
% \end{table*}


% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}

% \begin{table*}
% \centering
% \scriptsize
% \caption{Multivariate long-term forecasting results with MTST. Look back window $L=336$. We use prediction
% lengths $T \in \{96, 192, 336, 720\} $ all datasets. The best
% results are in \textbf{bold} and the second best are {\ul underlined}. Full results can be found in Appendix.
% \mlh{MTST/PatchTST/DLinear: $L=336$; Fedformer: best from $L=\{48, 96, 192, 336, 720\}$; TimesNet, MICN: $L=96$;
% PatchTST also has a version on $L=512$ with better results.
% To discuss whether this is a fair comparisons.}
% }
% \useunder{\uline}{\ul}{}
% % Please add the following required packages to your document preamble:
% % \usepackage{multirow}
% % \usepackage[normalem]{ulem}
% % \useunder{\uline}{\ul}{}
% \begin{tabular}{cc|cc|cc|cc|cc|cc|cc}
% \hline
% \multicolumn{2}{c|}{Models}                             & \multicolumn{2}{c|}{MTST}       & \multicolumn{2}{c|}{PatchTST} & \multicolumn{2}{c|}{TimesNet} & \multicolumn{2}{c|}{MICN} & \multicolumn{2}{c|}{Dlinear} & \multicolumn{2}{c}{Fedformer} \\ \hline
% \multicolumn{2}{c|}{Metric}                             & MSE            & MAE            & MSE             & MAE         & MSE           & MAE           & MSE         & MAE         & MSE         & MAE            & MSE           & MAE           \\ \hline
% \multicolumn{1}{c|}{\multirow{4}{*}{Traffic}}     & 96  & \textbf{0.353} & \textbf{0.238} & {\ul 0.367}     & {\ul 0.251} & 0.593         & 0.321         & 0.519       & 0.309       & 0.410       & 0.282          & 0.576         & 0.359         \\
% \multicolumn{1}{c|}{}                             & 192 & \textbf{0.378} & \textbf{0.253} & {\ul 0.385}     & {\ul 0.259} & 0.617         & 0.336         & 0.537       & 0.315       & 0.423       & 0.287          & 0.610         & 0.380         \\
% \multicolumn{1}{c|}{}                             & 336 & \textbf{0.386} & \textbf{0.258} & {\ul 0.398}     & {\ul 0.265} & 0.629         & 0.336         & 0.534       & 0.313       & 0.436       & 0.296          & 0.608         & 0.375         \\
% \multicolumn{1}{c|}{}                             & 720 & \textbf{0.425} & \textbf{0.281} & {\ul 0.434}     & {\ul 0.287} & 0.640         & 0.350         & 0.577       & 0.325       & 0.466       & 0.315          & 0.621         & 0.375         \\ \hline
% \multicolumn{1}{c|}{\multirow{4}{*}{Electricity}} & 96  & \textbf{0.128} & \textbf{0.222} & {\ul 0.130}     & {\ul 0.222} & 0.168         & 0.272         & 0.164       & 0.269       & 0.140       & 0.237          & 0.186         & 0.302         \\
% \multicolumn{1}{c|}{}                             & 192 & \textbf{0.144} & \textbf{0.238} & {\ul 0.148}     & {\ul 0.240} & 0.184         & 0.289         & 0.177       & 0.177       & 0.153       & 0.249          & 0.197         & 0.311         \\
% \multicolumn{1}{c|}{}                             & 336 & \textbf{0.162} & \textbf{0.256} & {\ul 0.167}     & {\ul 0.261} & 0.198         & 0.300         & 0.193       & 0.304       & 0.169       & 0.267          & 0.213         & 0.328         \\
% \multicolumn{1}{c|}{}                             & 720 & \textbf{0.199} & \textbf{0.289} & {\ul 0.202}     & {\ul 0.291} & 0.220         & 0.320         & 0.212       & 0.321       & 0.203       & 0.301          & 0.233         & 0.344         \\ \hline
% \multicolumn{1}{c|}{\multirow{4}{*}{Weather}}     & 96  & \textbf{0.150} & \textbf{0.199} & {\ul 0.152}     & {\ul 0.199} & 0.172         & 0.220         & 0.161       & 0.229       & 0.176       & 0.237          & 0.238         & 0.314         \\
% \multicolumn{1}{c|}{}                             & 192 & \textbf{0.194} & \textbf{0.240} & {\ul 0.197}     & {\ul 0.243} & 0.219         & 0.261         & 0.220       & 0.281       & 0.220       & 0.282          & 0.275         & 0.329         \\
% \multicolumn{1}{c|}{}                             & 336 & \textbf{0.246} & \textbf{0.281} & {\ul 0.249}     & {\ul 0.283} & 0.280         & 0.306         & 0.278       & 0.331       & 0.265       & 0.319          & 0.339         & 0.377         \\
% \multicolumn{1}{c|}{}                             & 720 & \textbf{0.319} & \textbf{0.333} & {\ul 0.320}     & {\ul 0.335} & 0.365         & 0.359         & 0.311       & 0.356       & 0.323       & 0.362          & 0.389         & 0.409         \\ \hline
% \multicolumn{1}{c|}{\multirow{4}{*}{ETTh1}}       & 96  & \textbf{0.358} & \textbf{0.390} & {\ul 0.375}     & {\ul 0.399} & 0.384         & 0.402         & 0.421       & 0.431       & {\ul 0.375} & {\ul 0.399}    & 0.376         & 0.415         \\
% \multicolumn{1}{c|}{}                             & 192 & \textbf{0.396} & \textbf{0.414} & 0.414           & 0.421       & 0.436         & 0.429         & 0.474       & 0.487       & {\ul 0.405} & {\ul 0.416}    & 0.423         & 0.446         \\
% \multicolumn{1}{c|}{}                             & 336 & \textbf{0.391} & \textbf{0.420} & {\ul 0.431}     & {\ul 0.436} & 0.491         & 0.469         & 0.569       & 0.551       & 0.439       & 0.443          & 0.444         & 0.462         \\
% \multicolumn{1}{c|}{}                             & 720 & \textbf{0.430} & \textbf{0.457} & {\ul 0.449}     & {\ul 0.466} & 0.521         & 0.500         & 0.770       & 0.672       & 0.472       & 0.490          & 0.469         & 0.492         \\ \hline
% \multicolumn{1}{c|}{\multirow{4}{*}{ETTh2}}       & 96  & \textbf{0.257} & \textbf{0.326} & {\ul 0.274}     & {\ul 0.336} & 0.340         & 0.374         & 0.299       & 0.364       & 0.289       & 0.353          & 0.332         & 0.374         \\
% \multicolumn{1}{c|}{}                             & 192 & \textbf{0.309} & \textbf{0.361} & {\ul 0.339}     & {\ul 0.379} & 0.402         & 0.414         & 0.441       & 0.454       & 0.383       & 0.418          & 0.407         & 0.446         \\
% \multicolumn{1}{c|}{}                             & 336 & \textbf{0.302} & \textbf{0.366} & {\ul 0.331}     & {\ul 0.380} & 0.452         & 0.452         & 0.654       & 0.567       & 0.448       & 0.465          & 0.400         & 0.447         \\
% \multicolumn{1}{c|}{}                             & 720 & \textbf{0.372} & \textbf{0.416} & {\ul 0.379}     & {\ul 0.422} & 0.462         & 0.468         & 0.956       & 0.716       & 0.605       & 0.551          & 0.412         & 0.469         \\ \hline
% \multicolumn{1}{c|}{\multirow{4}{*}{ETTm1}}       & 96  & \textbf{0.286} & \textbf{0.338} & {\ul 0.290}     & {\ul 0.342} & 0.338         & 0.375         & 0.316       & 0.362       & 0.299       & 0.343          & 0.326         & 0.390         \\
% \multicolumn{1}{c|}{}                             & 192 & \textbf{0.327} & {\ul 0.366}    & {\ul 0.332}     & 0.369       & 0.374         & 0.387         & 0.363       & 0.390       & 0.335       & \textbf{0.365} & 0.365         & 0.415         \\
% \multicolumn{1}{c|}{}                             & 336 & \textbf{0.362} & \textbf{0.389} & {\ul 0.366}     & {\ul 0.392} & 0.410         & 0.411         & 0.408       & 0.426       & 0.369       & 0.386          & 0.392         & 0.425         \\
% \multicolumn{1}{c|}{}                             & 720 & \textbf{0.414} & \textbf{0.421} & {\ul 0.420}     & {\ul 0.424} & 0.478         & 0.450         & 0.481       & 0.476       & 0.425       & \textbf{0.421} & 0.446         & 0.458         \\ \hline
% \multicolumn{1}{c|}{\multirow{4}{*}{ETTm2}}       & 96  & \textbf{0.162} & \textbf{0.251} & {\ul 0.165}     & {\ul 0.255} & 0.187         & 0.267         & 0.179       & 0.275       & 0.167       & 0.260          & 0.180         & 0.271         \\
% \multicolumn{1}{c|}{}                             & 192 & \textbf{0.220} & \textbf{0.291} & \textbf{0.220}  & {\ul 0.292} & 0.249         & 0.309         & 0.307       & 0.376       & {\ul 0.224} & 0.303          & 0.252         & 0.318         \\
% \multicolumn{1}{c|}{}                             & 336 & \textbf{0.276} & \textbf{0.329} & {\ul 0.278}     & {\ul 0.329} & 0.321         & 0.351         & 0.325       & 0.388       & 0.281       & 0.342          & 0.324         & 0.364         \\
% \multicolumn{1}{c|}{}                             & 720 & \textbf{0.358} & \textbf{0.379} & {\ul 0.367}     & {\ul 0.385} & 0.408         & 0.403         & 0.502       & 0.490       & 0.397       & 0.421          & 0.410         & 0.420        \\ \hline
% \end{tabular}
% \label{table:mtst}
% \end{table*}

\begin{table*}
\centering
\scriptsize
\caption{Multivariate long-term forecasting results with lookback window $L=336$ and prediction 
lengths $T \in \{96, 192, 336, 720\} $.
The best
results are in \textbf{bold} and the second best are \ul{underlined}.
% Full results can be found in Appendix.
Baseline results are from \cite{nie2023TimeSeriesWorth} and \cite{zeng2023AreTransformersEffective}.
% \mlh{MTST/PatchTST/DLinear: $L=336$; Fedformer: best from $L=\{48, 96, 192, 336, 720\}$; TimesNet, MICN: $L=96$;
% PatchTST also has a version on $L=512$ with better results.
% To discuss whether this is a fair comparisons.}
}
\label{tab:L336}
\useunder{\uline}{\ul}{}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}
\begin{tabular}{cc|cc|cc|cc|cc|cc|cc}
\hline
\multicolumn{2}{c|}{Models}                             & \multicolumn{2}{c|}{MTST}       & \multicolumn{2}{c|}{PatchTST} & \multicolumn{2}{c|}{Dlinear} & \multicolumn{2}{c|}{Fedformer}  & \multicolumn{2}{c|}{Autoformer} & \multicolumn{2}{c}{Informer}  \\ \hline
\multicolumn{2}{c|}{Metric}                             & MSE            & MAE            & MSE             & MAE         & MSE         & MAE            & MSE           & MAE            & MSE           & MAE             & MSE         & MAE          \\ \hline
\multicolumn{1}{c|}{\multirow{4}{*}{Traffic}}     & 96  & \textbf{0.353} & \textbf{0.238} & {\ul 0.367}     & {\ul 0.251} & 0.410       & 0.282          & 0.576         & 0.359          & 0.597         & 0.371           & 0.733       & 0.410        \\
\multicolumn{1}{c|}{}                             & 192 & \textbf{0.378} & \textbf{0.253} & {\ul 0.385}     & {\ul 0.259} & 0.423       & 0.287          & 0.610         & 0.380          & 0.607         & 0.382           & 0.777       & 0.435        \\
\multicolumn{1}{c|}{}                             & 336 & \textbf{0.386} & \textbf{0.258} & {\ul 0.398}     & {\ul 0.265} & 0.436       & 0.296          & 0.608         & 0.375          & 0.623         & 0.387           & 0.776       & 0.434        \\
\multicolumn{1}{c|}{}                             & 720 & \textbf{0.425} & \textbf{0.281} & {\ul 0.434}     & {\ul 0.287} & 0.466       & 0.315          & 0.621         & 0.375          & 0.639         & 0.395           & 0.827       & 0.466        \\ \hline
\multicolumn{1}{c|}{\multirow{4}{*}{Electricity}} & 96  & \textbf{0.128} & \textbf{0.222} & {\ul 0.130}     & {\ul 0.222} & 0.140       & 0.237          & 0.186         & 0.302          & 0.196         & 0.313           & 0.304       & 0.393        \\
\multicolumn{1}{c|}{}                             & 192 & \textbf{0.144} & \textbf{0.238} & {\ul 0.148}     & {\ul 0.240} & 0.153       & 0.249          & 0.197         & 0.311          & 0.211         & 0.324           & 0.327       & 0.417        \\
\multicolumn{1}{c|}{}                             & 336 & \textbf{0.162} & \textbf{0.256} & {\ul 0.167}     & {\ul 0.261} & 0.169       & 0.267          & 0.213         & 0.328          & 0.214         & 0.327           & 0.333       & 0.422        \\
\multicolumn{1}{c|}{}                             & 720 & \textbf{0.199} & \textbf{0.289} & {\ul 0.202}     & {\ul 0.291} & 0.203       & 0.301          & 0.233         & 0.344          & 0.236         & 0.342           & 0.351       & 0.427        \\ \hline
\multicolumn{1}{c|}{\multirow{4}{*}{Weather}}     & 96  & \textbf{0.150} & \textbf{0.199} & {\ul 0.152}     & {\ul 0.199} & 0.176       & 0.237          & 0.238         & 0.314          & 0.249         & 0.329           & 0.354       & 0.405        \\
\multicolumn{1}{c|}{}                             & 192 & \textbf{0.194} & \textbf{0.240} & {\ul 0.197}     & {\ul 0.243} & 0.220       & 0.282          & 0.275         & 0.329          & 0.325         & 0.370           & 0.419       & 0.434        \\
\multicolumn{1}{c|}{}                             & 336 & \textbf{0.246} & \textbf{0.281} & {\ul 0.249}     & {\ul 0.283} & 0.265       & 0.319          & 0.339         & 0.377          & 0.351         & 0.391           & 0.583       & 0.543        \\
\multicolumn{1}{c|}{}                             & 720 & \textbf{0.319} & \textbf{0.333} & {\ul 0.320}     & {\ul 0.335} & 0.323       & 0.362          & 0.389         & 0.409          & 0.415         & 0.426           & 0.916       & 0.705        \\ \hline
\multicolumn{1}{c|}{\multirow{4}{*}{ETTh1}}       & 96  & \textbf{0.358} & \textbf{0.390} & {\ul 0.375}     & {\ul 0.399} & {\ul 0.375} & {\ul 0.399}    & 0.376         & 0.415          & 0.435         & 0.446           & 0.941       & 0.760        \\
\multicolumn{1}{c|}{}                             & 192 & \textbf{0.396} & \textbf{0.414} & 0.414           & 0.421       & {\ul 0.405} & {\ul 0.416}    & 0.423         & 0.446          & 0.456         & 0.457           & 1.007       & 0.786        \\
\multicolumn{1}{c|}{}                             & 336 & \textbf{0.391} & \textbf{0.420} & {\ul 0.431}     & {\ul 0.436} & 0.439       & 0.443          & 0.444         & 0.462          & 0.486         & 0.487           & 1.038       & 0.784        \\
\multicolumn{1}{c|}{}                             & 720 & \textbf{0.430} & \textbf{0.457} & {\ul 0.449}     & {\ul 0.466} & 0.472       & 0.490          & 0.469         & 0.492          & 0.515         & 0.517           & 1.144       & 0.857        \\ \hline
\multicolumn{1}{c|}{\multirow{4}{*}{ETTh2}}       & 96  & \textbf{0.257} & \textbf{0.326} & {\ul 0.274}     & {\ul 0.336} & 0.289       & 0.353          & 0.332         & 0.374          & 0.332         & 0.368           & 1.549       & 0.952        \\
\multicolumn{1}{c|}{}                             & 192 & \textbf{0.309} & \textbf{0.361} & {\ul 0.339}     & {\ul 0.379} & 0.383       & 0.418          & 0.407         & 0.446          & 0.426         & 0.434           & 3.792       & 1.542        \\
\multicolumn{1}{c|}{}                             & 336 & \textbf{0.302} & \textbf{0.366} & {\ul 0.331}     & {\ul 0.380} & 0.448       & 0.465          & 0.400         & 0.447          & 0.477         & 0.477           & 4.215       & 1.642        \\
\multicolumn{1}{c|}{}                             & 720 & \textbf{0.372} & \textbf{0.416} & {\ul 0.379}     & {\ul 0.422} & 0.605       & 0.551          & 0.412         & 0.469          & 0.453         & 0.453           & 3.656       & 1.619        \\ \hline
\multicolumn{1}{c|}{\multirow{4}{*}{ETTm1}}       & 96  & \textbf{0.286} & \textbf{0.338} & {\ul 0.290}     & {\ul 0.342} & 0.299       & 0.343          & 0.326         & 0.390          & 0.510         & 0.492           & 0.626       & 0.560        \\
\multicolumn{1}{c|}{}                             & 192 & \textbf{0.327} & {\ul 0.366}    & {\ul 0.332}     & 0.369       & 0.335       & \textbf{0.365} & 0.365         & 0.415          & 0.514         & 0.495           & 0.725       & 0.619        \\
\multicolumn{1}{c|}{}                             & 336 & \textbf{0.362} & \textbf{0.389} & {\ul 0.366}     & {\ul 0.392} & 0.369       & 0.386          & 0.392         & 0.425          & 0.510         & 0.492           & 1.005       & 0.741        \\
\multicolumn{1}{c|}{}                             & 720 & \textbf{0.414} & \textbf{0.421} & {\ul 0.420}     & {\ul 0.424} & 0.425       & \textbf{0.421} & 0.446         & 0.458          & 0.453         & 0.493           & 1.133       & 0.845        \\ \hline
\multicolumn{1}{c|}{\multirow{4}{*}{ETTm2}}       & 96  & \textbf{0.162} & \textbf{0.251} & {\ul 0.165}     & {\ul 0.255} & 0.167       & 0.260          & 0.180         & 0.271          & 0.205         & 0.293           & 0.355       & 0.462        \\
\multicolumn{1}{c|}{}                             & 192 & \textbf{0.220} & \textbf{0.291} & \textbf{0.220}  & {\ul 0.292} & {\ul 0.224} & 0.303          & 0.252         & 0.318          & 0.278         & 0.336           & 0.595       & 0.586        \\
\multicolumn{1}{c|}{}                             & 336 & \textbf{0.276} & \textbf{0.329} & {\ul 0.278}     & {\ul 0.329} & 0.281       & 0.342          & 0.324         & 0.364          & 0.343         & 0.379           & 1.270       & 0.871        \\
\multicolumn{1}{c|}{}                             & 720 & \textbf{0.358} & \textbf{0.379} & {\ul 0.367}     & {\ul 0.385} & 0.397       & 0.421          & 0.410         & 0.420          & 0.414         & 0.419           & 3.001       & 1.267       \\ \hline
\end{tabular}
\label{table:mtst}
\end{table*}







\begin{table*}
\centering
\scriptsize
\caption{Multivariate long-term forecasting results with MTST. Look back window $L=96$ and prediction
lengths $T \in \{96, 192, 336, 720\} $.
The best
results are in {bold} and the second best are {\ul underlined}.
The baseline results are from the original paper except PatchTST, which we reproduce for $L=96$.
\mlh{To update the result for MTST and PatchTST for $L=96$}
}\label{tab:L96}
\useunder{\uline}{\ul}{}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}
\begin{tabular}{cc|cc|cc|cc|cc|cc|cc}
\hline
\multicolumn{2}{c|}{Models}                             & \multicolumn{2}{c|}{MTST}        & \multicolumn{2}{c|}{PatchTST}  & \multicolumn{2}{c|}{TimesNet}  & \multicolumn{2}{c|}{Crossformer}  & \multicolumn{2}{c|}{MICN}   & \multicolumn{2}{c}{Scaleformer}     \\ \hline
\multicolumn{2}{c|}{Metric}                             & MSE            & MAE             & MSE             & MAE             & MSE           & MAE            & MSE           & MAE              & MSE         & MAE           & MSE         & MAE                   \\ \hline
\multicolumn{1}{c|}{\multirow{4}{*}{Traffic}}     & 96  & {0.426} & {0.275}  & -               & -               & 0.593         & 0.321          & -             & -                & 0.519       & 0.309         & 0.564       & 0.351                 \\
\multicolumn{1}{c|}{}                             & 192 & {-    } & {-    }  & -               & -               & 0.617         & 0.336          & -             & -                & 0.537       & 0.315         & 0.570       & 0.349                 \\
\multicolumn{1}{c|}{}                             & 336 & {0.451} & {0.284}  & -               & -               & 0.629         & 0.336          & 0.530         & 0.300            & 0.534       & 0.313         & 0.576       & 0.349                 \\
\multicolumn{1}{c|}{}                             & 720 & {0.482} & {0.302}  & -               & -               & 0.640         & 0.350          & 0.573         & 0.313            & 0.577       & 0.325         & 0.602       & 0.360                 \\ \hline
\multicolumn{1}{c|}{\multirow{4}{*}{Electricity}} & 96  & {0.166} & {0.252}  & -               & -               & 0.168         & 0.272          & -             & -                & 0.164       & 0.269         & 0.182       & 0.297                 \\
\multicolumn{1}{c|}{}                             & 192 & {0.175} & {0.262}  & -               & -               & 0.184         & 0.289          & -             & -                & 0.177       & 0.177         & 0.188       & 0.300                 \\
\multicolumn{1}{c|}{}                             & 336 & {0.191} & {0.278}  & -               & -               & 0.198         & 0.300          & 0.404         & 0.423            & 0.193       & 0.304         & 0.210       & 0.324                 \\
\multicolumn{1}{c|}{}                             & 720 & {-----} & {-----}  & -               & -               & 0.220         & 0.320          & 0.433         & 0.438            & 0.212       & 0.321         & 0.232       & 0.339                 \\ \hline
\multicolumn{1}{c|}{\multirow{4}{*}{Weather}}     & 96  & {0.177} & {0.215}  & -               & -               & 0.172         & 0.220          & -             & -                & 0.161       & 0.229         & 0.163       & 0.226                 \\
\multicolumn{1}{c|}{}                             & 192 & {0.223} & {0.256}  & -               & -               & 0.219         & 0.261          & -             & -                & 0.220       & 0.281         & 0.221       & 0.290                 \\
\multicolumn{1}{c|}{}                             & 336 & {0.277} & {0.296}  & -               & -               & 0.280         & 0.306          & 0.495         & 0.515            & 0.278       & 0.331         & 0.282       & 0.340                 \\
\multicolumn{1}{c|}{}                             & 720 & {0.352} & {0.347}  & -               & -               & 0.365         & 0.359          & 0.526         & 0.542            & 0.311       & 0.356         & 0.369       & 0.396                 \\ \hline
\multicolumn{1}{c|}{\multirow{4}{*}{ETTh1}}       & 96  & {0.374} & {0.391}  & -               & -               & 0.384         & 0.402          & -             & -                & 0.421       & 0.431         & -           & -                     \\
\multicolumn{1}{c|}{}                             & 192 & {0.430} & {0.420}  & -               & -               & 0.436         & 0.429          & -             & -                & 0.474       & 0.487         & -           & -                     \\
\multicolumn{1}{c|}{}                             & 336 & {0.447} & {0.434}  & -               & -               & 0.491         & 0.469          & 0.440         & 0.461            & 0.569       & 0.551         & -           & -                     \\
\multicolumn{1}{c|}{}                             & 720 & {0.460} & {0.461}  & -               & -               & 0.521         & 0.500          & 0.519         & 0.524            & 0.770       & 0.672         & -           & -                     \\ \hline
\multicolumn{1}{c|}{\multirow{4}{*}{ETTh2}}       & 96  & {0.275} & {0.332}  & -               & -               & 0.340         & 0.374          & -             & -                & 0.299       & 0.364         & -           & -                     \\
\multicolumn{1}{c|}{}                             & 192 & {0.347} & {0.377}  & -               & -               & 0.402         & 0.414          & -             & -                & 0.441       & 0.454         & -           & -                     \\
\multicolumn{1}{c|}{}                             & 336 & {0.359} & {0.396}  & -               & -               & 0.452         & 0.452          & -             & -                & 0.654       & 0.567         & -           & -                     \\
\multicolumn{1}{c|}{}                             & 720 & {0.407} & {0.431}  & -               & -               & 0.462         & 0.468          & -             & -                & 0.956       & 0.716         & -           & -                     \\ \hline
\multicolumn{1}{c|}{\multirow{4}{*}{ETTm1}}       & 96  & {0.324} & {0.361}  & -               & -               & 0.338         & 0.375          & -             & -                & 0.316       & 0.362         & -           & -                     \\
\multicolumn{1}{c|}{}                             & 192 & {0.364} & {0.386}  & -               & -               & 0.374         & 0.387          & -             & -                & 0.363       & 0.390         & -           & -                     \\
\multicolumn{1}{c|}{}                             & 336 & {0.392} & {0.406}  & -               & -               & 0.410         & 0.411          & 0.404         & 0.427            & 0.408       & 0.426         & -           & -                     \\
\multicolumn{1}{c|}{}                             & 720 & {0.451} & {0.439}  & -               & -               & 0.478         & 0.450          & 0.569         & 0.528            & 0.481       & 0.476         & -           & -                     \\ \hline
\multicolumn{1}{c|}{\multirow{4}{*}{ETTm2}}       & 96  & {0.177} & {0.260}  & -               & -               & 0.187         & 0.267          & -             & -                & 0.179       & 0.275         & -           & -                     \\
\multicolumn{1}{c|}{}                             & 192 & {0.248} & {0.306}  & -               & -               & 0.249         & 0.309          & -             & -                & 0.307       & 0.376         & -           & -                     \\
\multicolumn{1}{c|}{}                             & 336 & {0.309} & {0.344}  & -               & -               & 0.321         & 0.351          & -             & -                & 0.325       & 0.388         & -           & -                     \\
\multicolumn{1}{c|}{}                             & 720 & {0.403} & {0.396}  & -               & -               & 0.408         & 0.403          & -             & -                & 0.502       & 0.490         & -           & -                    \\ \hline
\end{tabular}
\label{table:mtst}
\end{table*}



% \begin{figure}
%     \centering
%     \includegraphics[width=1\linewidth]{Figure/360_var11_layers.pdf}
%     \caption{MTST: Electricity 720 branch visualization - \yitian{Reprint with larger label and text}}
%     \label{fig:mtst_elc_720}
% \end{figure}

% \begin{figure}
%     \centering
%     \includegraphics[width=0.8\linewidth]{Figure/360_var11_attns.pdf}
%     \caption{MTST: Electricity 720 attention map}
%     \label{fig:mtst_elc_720}
% \end{figure}

%put all figures here
% \input{Sections/visualize}


\mlh{To update after getting the final results}

Table~\ref{tab:L336} shows the main experimental results of all methods for eight datasets on MSE and MAE, where the best and second-best results for each case (dataset, horizon, and metric) are highlighted in bold and underlined, respectively.
MTST showcases a notable improvement in accuracy in 29 out of 32 cases when compared to the best existing method, PatchTST, at a look-back window of $L=336$. This achievement stands in stark contrast to DLinear, which cast doubts on the efficacy of transformers in Multivariate Time Series forecasting. MTST demonstrates a substantial reduction of 11.92\% in MSE and 9.75\% in MAE.


Table~\ref{tab:L96}

In comparison to the multi-scale Convolutional Neural Network (CNN)-based approach, MICN, MTST exhibits an average enhancement of 24.22\% in MSE and 16.36\% in MAE. Furthermore, when evaluated against the transformer-based multi-scale method Crossformer, MTST showcases a remarkable reduction in MSE and MAE by averages of 39.14\% and 28.49\%, respectively. These results underscore the superior performance of MTST, highlighting its effectiveness in improving forecasting accuracy in diverse scenarios.



\subsection{Ablation Study}
\subsubsection{How important is the multi-resolution design?}
Figure.\ref{fig:patch_len} shows that MSE scores vary with different
choices of $P$, and that there is no clear trend showing a consistent relationship between patch length and performance. It is a common phenomenon especially when dealing with complex and dynamic datasets like time series. It underscores several important principles and challenges:
First, time series data often exhibit complex temporal dependencies and patterns. Different patch sizes may be more or less effective at capturing specific temporal information, depending on the nature of these patterns. As a result, there might not be a one-size-fits-all patch size that consistently outperforms others.
Second,  the choice of patch size often involves trade-offs. Smaller patches may excel at capturing short-term fluctuations but miss long-term trends, while larger patches may capture broader trends but lose sensitivity to finer details. 

Our proposed model which involve analyzing data at multiple resolutions imultaneously, can indeed be effective in capturing diverse temporal patterns and improving model robustness.

By considering multiple temporal resolutions or patch sizes, we can capture a wide range of temporal patterns, from short-term fluctuations to long-term trends. This comprehensive view of the data can lead to more accurate and robust models.

\yitian{Branch-wise decomposition along with patch-TST comparison.}

% Figure. is the visualization of the prediction of each branch at last layer, which could serves as compelling evidence that our multi-resolution structure excels at capturing diverse patterns within the data. This experiment is conducted on Electricity dataset, with patch length [8, 32, 96] in each branch. From the figure, we can see that each branch within the architecture demonstrates a unique ability to capture and represent distinct temporal features. For example, the last branch with $P=96$ is mainly capturing the weekly pattern, where we can see from the ground truth that there is an electricity comsumption decay on the weekend. 

% thereby highlighting the efficacy of our model in capturing a wide range of information. for 



% Reduced Overfitting: Multi-resolution techniques can help mitigate overfitting issues that may arise when using a single fixed patch size. Models that generalize well across different resolutions are less prone to memorizing noise. see figure 4.

% Enhanced Interpretability: Multi-resolution analyses can provide insights into the presence and characteristics of temporal patterns at various scales. This can be valuable for understanding the underlying dynamics of your time series. see figure 5

% Improved Forecasting: Multiscale models can lead to more accurate and reliable forecasts, as they are less likely to miss important temporal features. see table 2.



\begin{figure}[htbp]
\centering
\includegraphics[width=0.9\linewidth]{Figure/patch_size.png}
\caption{MSE scores with varying patch lengths P = [2, 4, 8, 12, 16, 24, 32, 40] where the lookback window is 336 and the prediction length is 96}
\label{fig:patch_len}
\end{figure}


\subsubsection{How important is the relative positional encoding?}
Table. \ref{table:PE} shows the effect of positional encoding. From the table we can see that the Relative positional encodings (RPE) exhibit good utility and effectiveness, achieving 1.91\% performance improvement when applied to traffic dataset and 4.52\% on ETTh2 dataset, \yitian{compared to non-PE setting}. 

\yitian{Plot attn map of PatchTST and MTST(RPE) – MTST(RPE) shows more power on capturing periodic information than Patch.
}
% Figure.~, the visualization of attention map from Electricity also shows that the incorporation of relative positional encoding (RPE) enhances our model's ability to capture periodicity within time series data. Relative PE not only aids in identifying periodic patterns but also makes a valuable contribution to the overall score or performance metric, underscoring its significance in our approach.


\begin{table} 
\tiny
\centering
\caption{Multivariate long-term forecasting results of MTST with different positional encoding method. Look back window $L=336$. The best
results are in \textbf{bold} and the second best are {\ul underlined}}.
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
% \usepackage[normalem]{ulem}
\useunder{\uline}{\ul}{}
\begin{tabular}{c|c|cc|cc|cc}
\multicolumn{2}{c|}{Models}     & \multicolumn{2}{c|}{MTST (no RPE)}              & \multicolumn{2}{c|}{MTST (APE)}  & \multicolumn{2}{c}{MTST}    \\ \hline
\multicolumn{2}{c|}{Metric}     & MSE& MAE& MSE& MAE& MSE& MAE\\ \hline
                          Traffic& 96& 0.364& 0.248&{\ul0.354} & {\ul0.244} & \textbf{0.353}& \textbf{0.238}
\\
                          & 192& 0.382& \textbf{0.259}& {\ul0.382}& 0.265& \textbf{0.380}& {\ul0.261}
\\
                              & 336& 0.393& 0.263& {\ul0.387}& {\ul0.260}&\textbf{0.386}& \textbf{0.258}
\\
& 720& 0.435& 0.287& 0.426& 0.284& \textbf{0.425}& \textbf{0.281}
\\ \hline
                          ETTh2& 96& {\ul0.260}& 0.324& 0.268& 0.332& \textbf{0.259}& \textbf{0.324}
\\
                              & 192& 0.339& 0.383& {\ul0.334}& {\ul0.379}& \textbf{0.316}& \textbf{0.364}
\\
                          & 336& 0.330& 0.385& {\ul0.324}& {\ul0.380}&\textbf{0.309}& \textbf{0.369}
\\
& 720& 0.395& 0.437& {\ul0.392}& {\ul0.430}& \textbf{0.377}& \textbf{0.421}
\end{tabular}
\label{table:PE}
\end{table}

% \begin{figure}
%     \centering
%     \includegraphics[width=1\linewidth]{Figure/360_var11_attns.pdf}
%     \caption{MTST: Electricity 720 attention map, \soumya{need bigger captions and axis markers}}
%     \label{fig:mtst_elc_720}
% \end{figure}

\subsubsection{Influence of branch number and layer number}
Figure.~\ref{fig:brach_layer} shows the effect of the number of branches and layers on an examples Etth2 and Ettm2 datasets. The analysis reveals that single-layer models exhibit lower capability in comparison to those with multiple layers. However, an issue of overfitting arises when increasing the number of layers from 2 to 3. Notably, for 1 and 2-layer MTST in the etth1 dataset, there is a discernible trend: with a higher branch number, the model performs better. In the Ettm2 dataset, the model achieves its best results with 2 branches. This variance in optimal branch numbers across datasets is logical, considering that each dataset focuses on distinct frequency bands.

\begin{figure}
    \centering
         \begin{subfigure}[b]{0.48\textwidth}
         \centering
        \includegraphics[width=1\linewidth]{Figure/abl/etth2br_new.png}
    \caption{Etth2}
     \end{subfigure}
\hfill
     \begin{subfigure}[b]{0.5\textwidth}
         \centering
        \includegraphics[width=1\linewidth]{Figure/abl/ETTm1br.png}
    \caption{Ettm2}
     \end{subfigure}
%      \begin{subfigure}[b]{0.5\textwidth}
%          \centering
%         \includegraphics[width=1\linewidth]{Figure/abl/ETTh1br.png}
%     \caption{Etth1}
%      \end{subfigure}
% \hfill

\caption{\yitian{Figures will be replot}Effect of number of branches and layers on different datasets. Lookback window $L = 336$, horizon $T = 336$ }
\label{fig:brach_layer}
\end{figure}

\subsubsection{Influence of look back window}
The size of the input sequence plays a crucial role in MTS forecasting as it determines the amount of historical information that can be utilized. Theoretically, an extended input sequence is expected to enhance forecasting accuracy as it encompasses a greater volume of information. However, recent studies have shown that this assumption does not always hold. Figure 4 illustrates the effect of the input sequence length on the forecasting accuracy. Take etth1 as an example, when averaging the MSE of all horizons, the performance gets better when the input sequence becomes longer. Moreover, MTST demonstrates greater improvement compared to patchTST when the look-back window is shorter.

% \yitian{Conclusion will be made after more case studies. Might be: 1)the optimal input sequence length varies depending on the dataset and forecasting horizon. 2)performance and $L$ is positive correlative.}

\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{Figure/etth_Lookback_window.png}
    \caption{Effect of size of look back window, with 2 layers and 2 branches. Reported MSE is average of horizons T = \{96, 192, 336, 700\} }
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{Figure/abl/lookback.png}
    \caption{Effect of size of look back window}
\end{figure}

% From Table.\ref{MTST_abs} we can see that:
% a) Relative positional encodings (PE) exhibit greater utility and effectiveness when applied to traffic datasets compared to other datasets. The reason is that Relative Positional Encodings (RPE) prove to be more valuable in situations where a higher degree of periodicity is present.

% b) L2 attention has a relatively smaller contribution to the final results. The first reason could be the transformer structure is not useful for small time series datasets, since it could be over-fitting during training. In previous experiments, we also showed that when K and Q are set to 0, we had similar results compared to baseline. The second reason of L2 is not effective as we expected is that these datasets are not in the same pattern as we proposed in Figure.4, --patches have the same wavelength but different scales. In this case, it makes sense that the L2 attention is not working properly on these datasets.

% To do: \\
% a) analyze how MTST structure helps.\\
% b) Parameter tuning for all datasets.\\
% c) Experiments on overlapping patches. \\

% \begin{figure}
%     \centering
%     \includegraphics[width=\linewidth]{Figure/paralMTST.png}
%     \caption{Ablation Study. \\
%     PatchTST:baseline. \\
%     PatchTST + RPE: replace absolute PE with relative PE. \\
%     PatchTST(l2): replace dot-produce with l2 attn. \\
%     PatchTST(l2)+RPE: replace dot-produce with l2 attn, plus relative PE. \\
%     MTST(l2)+RPE: the MTST proposed in Section.2.\\
%     (One more column: only MTST structure)}
%     \label{MTST_abs}
% \end{figure}


==> sections/old_version/introduction.tex <==


\section{INTRODUCTION}
\label{section:intro}


Multivariate time series forecasting, the process of predicting multiple variables over time, is a critical task in various domains such as finance, weather prediction, energy management, and healthcare. With the swift expansion of deep learning methodologies, research endeavors in this realm have surged notably. [some survey refernece]. 

% \yitian{add ref from other domain}
The Transformer model has emerged as a highly successful architecture in diverse fields such as natural language processing (NLP), computer vision (CV) , speech. Its effectiveness stems from the attention mechanism, allowing it to autonomously learn relationships between elements in a sequence, making it particularly suited for sequential modeling tasks. 
In previous years, variants like Informer~\cite{zhou2021InformerEfficientTransformer}, Autoformer~\cite{wu2021AutoformerDecompositionTransformers}, and FEDformer~\cite{zhou2022FEDformerFrequencyEnhanced} have demonstrated the Transformer's prowess in handling time series data. However, a study~\cite{zeng2023AreTransformersEffective} showed that a remarkably simple linear model could outperform all previous models across several common benchmarks. This challenges the perceived utility of the Transformer architecture in the realm of time series forecasting. 


Most recently, PatchTST~\cite{nie2022TimeSeiresWorth} and Crossformer~\cite{zhang2022crossformerTransformerUtilizing} have introduced a patching technique where each series in Multivariate Time Series (MTS) data is divided into specific-length patches. This approach allows the utilization of a standard transformer to capture temporal dependencies at the sub-series level.


\mlh{To consider changing the way to tell the story for multiscale; 
Alternatively: 1. introduce the necessity of multi-scale learning;
2. show that in patch-based Transformers, the token size is related to the multi-scale/multi-resolution;
3. propose the multi-branch multi-resolution via self-attentions with different token sizes (via reshaping) 
}


\mlh{Add the figure comparing patch-size in PatchTST to support our motivation.
}

However, there is no clear trend showing a consistent relationship between patch length and performance~\cite{nie2023TimeSeriesWorth}. It is a common phenomenon especially when dealing with complex and dynamic datasets like time series. It underscores several important principles and challenges:
First, time series data often exhibit complex temporal dependencies and patterns. Different patch sizes may be more or less effective at capturing specific temporal information, depending on the nature of these patterns. As a result, there might not be a one-size-fits-all patch size that consistently outperforms others.
Second, the choice of patch size often involves trade-offs. Smaller patches may excel at capturing short-term fluctuations but miss long-term trends, while larger patches may capture broader trends but lose sensitivity to finer details. 
Therefore, we propose the Multi-resolution Transformer for long-term time series forecasting (MTST), in which each branch focuses on a different granularity of the time series. 

\mlh{To add the main figure similar to ~\ref{fig:main_fig}}.

\begin{figure}[h!]
    \centering
    \includegraphics[width=0.5\textwidth]{Figure/others/convNext.png}
    \caption{\mlh{To add a main figure similar to this figure}}
    \label{fig:main_fig}
\end{figure}


% Our contributions can be summarized as follows:


% It is generally known that Transformers~\cite{vaswani2017AttentionAllYou, dosovitskiy2020ImageWorth16x16} lack \textit{strong inductive bias}.
% Unexceptionally on time series forecasting, a recent study~\cite{zeng2023AreTransformersEffective} has also revealed that transformers perform unsatisfactorily due to the failure to capture the sequential information of the time steps, which is a strong inductive bias on time series forecasting.
% In this work, we aim to show that, by injecting proper inductive biases, transformers are effective and powerful in time series forecasting.

% Unlike natural language and computer vision domains, the locality is not the (only) valid inductive bias in time series forecasting.
% Instead, seasonal patterns with different wavelengths, corresponding to the frequency patterns, have been emphasized by several works as a strong inductive bias on time series
% % (shown in Figure.~\ref{fig:freq_decopose}). 
% \cite{zeng2023AreTransformersEffective} introduces two types of preprocessing techniques, subtraction-based normalization and seasonal-trend decomposition, to enhance the linear models on time series forecasting.
% \textit{NHits}~\cite{challu2022NHiTSNeuralHierarchical} proposes to assemble the predictions sequentially as interpolation, emphasizing components with different wavelengths and scales from the time domain.
% \textit{Fedformer}~\cite{zhou2022FEDformerFrequencyEnhanced}, proposes to introduce the Fourier Transforms into the attention mechanism to better capture the frequency information from the frequency domain.


% It is worth mentioning that, using the \text{de facto} standard absolute \textit{sinusoidal positional encoding} (SinPE) on the vanilla Transformers (scaled dot-product attention)~~\cite{vaswani2017AttentionAllYou} cannot effectively explore the frequency patterns 
% (shown in Sec.~\ref{par:sinpe}).

% \begin{figure}[h!]
%     \centering
%     \includegraphics[width=0.8\textwidth]{figures/nhits.png}
%     \caption{The illustration of frequency decomposition. Figure taken from NHits~\cite{challu2022NHiTSNeuralHierarchical}}
%     \label{fig:freq_decopose}
% \end{figure}
